Dynamic Pricing for Airline Ancillaries with Customer Context

Ancillaries have become a major source of revenue and profitability in the travel industry. Yet, conventional pricing strategies are based on business rules that are poorly optimized and do not respond to changing market conditions. This paper describes the dynamic pricing model developed by Deepair solutions, an AI technology provider for travel suppliers. We present a pricing model that provides dynamic pricing recommendations specific to each customer interaction and optimizes expected revenue per customer. The unique nature of personalized pricing provides the opportunity to search over the market space to find the optimal price-point of each ancillary for each customer, without violating customer privacy. In this paper, we present and compare three approaches for dynamic pricing of ancillaries, with increasing levels of sophistication: (1) a two-stage forecasting and optimization model using a logistic mapping function; (2) a two-stage model that uses a deep neural network for forecasting, coupled with a revenue maximization technique using discrete exhaustive search; (3) a single-stage end-to-end deep neural network that recommends the optimal price. We describe the performance of these models based on both offline and online evaluations. We also measure the real-world business impact of these approaches by deploying them in an A/B test on an airline's internet booking website. We show that traditional machine learning techniques outperform human rule-based approaches in an online setting by improving conversion by 36% and revenue per offer by 10%. We also provide results for our offline experiments which show that deep learning algorithms outperform traditional machine learning techniques for this problem. Our end-to-end deep learning model is currently being deployed by the airline in their booking system.

==> sections/egreedyapproach.tex <==
\section{\(\bm{\epsilon}\)-greedy approach} \akcomment{This should be its own section}
Estimating the actual demand curve \(D(P, \theta)\) is significantly challenging and directly maximizing expected revenue often fails to produce practical results. More importantly, to accurately model ancillary purchase probability distribution without the ground truth information about purchase on variable prices is extremely challenging. Hence, we used a \(\epsilon\)-greedy approach to overcome the accurate estimation hurdle. First, a model is trained offline to predict the probability of purchase for the offered ancillary at a given price. Along with logistic model which maps probabilities to price, this model is set to explore online to collect experience and gain information about price sensitivity for a given ancillary. Then, the model chooses logistic exploration with probability \(\epsilon\) and revenue maximization with probability \(1 - \epsilon\).

\begin{equation} \label{eq:epsgreedy}
P^{rec} = \begin{cases}
P^{log} & \text{s.t. \(p<\epsilon\)}\\
P^{rm} &\text{otherwise}
\end{cases}
\end{equation}

This approach enables us to estimate customers' elasticity towards variable ancillary price by using an alias of the probability of selection $f$, as demand function $D$.

We used Gaussian Naive Bayes (GNB) as a baseline model \akcomment{not sure if we can refer to it as a 'baseline'}  for predicting ancillary selection probability. Random forest (RF) and Gradient Boasting Machine (GBM) models' performances are also compared. Finally, a deep neural network (DNN) is an ancillary selection model.

The ad-hoc loss function used to train the model based on discrete exhaustive search is inspired from regression model used in Airbnb pricing and SVR \cite{haldar2018applying, smola2004tutorial}. However, our overall loss function uses \(\epsilon\)-greedy approach and operates on discrete search space. 
